A planar algebra construction of the Haagerup subfactor

Most known examples of subfactors occur in families, coming from algebraic objects such as groups, quantum groups and rational conformal field theories. The Haagerup subfactor is the smallest index finite-depth subfactor which does not occur in one of these families. In this paper we construct the planar algebra associated to the Haagerup subfactor, which provides a new proof of the existence of the Haagerup subfactor. Our technique is to find the Haagerup planar algebra as a singly generated subfactor planar algebra, contained inside of a graph planar algebra.

==> Diagrams/AlphaITensorStrand.tex <==
\begin{tikzpicture}[scale=.3,baseline=-1mm]
	\draw (-1.5,-1) rectangle (1.5,1);
	\node at (0,0) {$\alpha_i$};
	\draw (-1,-1)--(-1,-1.5);
	\node at (0,1.25) {...};
	\draw (1,-1)--(1,-1.5);
	\draw (-1,1)--(-1,1.5);
	\node at (0,-1.25) {...};
	\draw (1,1)--(1,1.5);
	\draw (2,-1.5)--(2,1.5);
\end{tikzpicture}

==> Diagrams/AlphaTensorStrand.tex <==
\begin{tikzpicture}[scale=.3,baseline=-1mm]
	\draw (-1.5,-1) rectangle (1.5,1);
	\node at (0,0) {$\alpha$};
	\draw (-1,-1)--(-1,-1.5);
	\node at (0,1.25) {...};
	\draw (1,-1)--(1,-1.5);
	\draw (-1,1)--(-1,1.5);
	\node at (0,-1.25) {...};
	\draw (1,1)--(1,1.5);
	\draw (2,-1.5)--(2,1.5);
\end{tikzpicture}

==> Diagrams/Generator/Cap.tex <==
\begin{tikzpicture}[annular]
	\clip (0,0) circle (2cm);

	\filldraw[shaded] (0,0)--(158:1cm) .. controls ++(158:1cm) and ++(112:1cm) .. (112:1cm) -- (0,0);
	\filldraw[shaded] (0,0)--(-158:2cm) arc (-158:-112:2cm) -- (0,0);
	\filldraw[shaded] (0,0)--(22:2cm) arc (22:68:2cm) -- (0,0);
	\filldraw[shaded] (0,0)--(-22:2cm) arc (-22:-68:2cm) -- (0,0);
		
	\draw[ultra thick] (0,0) circle (2cm);
	
	\node at (0,0)  [Tbox] (T) {$T$};
	\node at (T.180) [left] {$\star$};
	\node at (180:2cm) [right] {$\star$};
\end{tikzpicture}
=
\begin{tikzpicture}[annular]
	\clip (0,0) circle (2cm);

	\filldraw[shaded] (0,0)--(158:2cm) arc (158:22:2cm) -- (0,0) -- (68:1cm) .. controls ++(68:1cm) and ++(112:1cm) .. (112:1cm) -- (0,0);
	\filldraw[shaded] (0,0)--(-158:2cm) arc (-158:-112:2cm) -- (0,0);
	\filldraw[shaded] (0,0)--(-22:2cm) arc (-22:-68:2cm) -- (0,0);
		
	\draw[ultra thick] (0,0) circle (2cm);
		
	\node at (0,0)  [Tbox] (T) {$T$};
	\node at (T.180) [left] {$\star$};
	\node at (180:2cm) [right] {$\star$};
\end{tikzpicture}
=0

==> Diagrams/Generator/Cap1.tex <==
\begin{tikzpicture}[annular]
\begin{scope}
	\clip (0,0) circle (2cm);

	\filldraw[shaded] (0,0)--(158:1cm) .. controls ++(158:1cm) and ++(112:1cm) .. (112:1cm) -- (0,0);
	\filldraw[shaded] (0,0)--(-158:2cm) arc (-158:-112:2cm) -- (0,0);
	\filldraw[shaded] (0,0)--(22:2cm) arc (22:68:2cm) -- (0,0);
	\filldraw[shaded] (0,0)--(-22:2cm) arc (-22:-68:2cm) -- (0,0);
		
	\draw[ultra thick] (0,0) circle (2cm);
	
	\node at (0,0)  [Tbox] (T) {$T$};
	\node at (T.180) [left] {$\star$};
\end{scope}
	\node at (180:2cm) [left] {$\star$};
\end{tikzpicture}

==> Diagrams/Generator/Cap2.tex <==
\begin{tikzpicture}[annular]
\begin{scope}
	\clip (0,0) circle (2cm);

	\filldraw[shaded] (0,0)--(158:2cm) arc (158:22:2cm) -- (0,0) -- (68:1cm) .. controls ++(68:1cm) and ++(112:1cm) .. (112:1cm) -- (0,0);
	\filldraw[shaded] (0,0)--(-158:2cm) arc (-158:-112:2cm) -- (0,0);
	\filldraw[shaded] (0,0)--(-22:2cm) arc (-22:-68:2cm) -- (0,0);
		
	\draw[ultra thick] (0,0) circle (2cm);
		
	\node at (0,0)  [Tbox] (T) {$T$};
	\node at (T.180) [left] {$\star$};
\end{scope}
	\node at (180:2cm) [left] {$\star$};
\end{tikzpicture}

==> Diagrams/Generator/DoubleCircle.tex <==
\begin{tikzpicture}[annular]
	\clip (0,0) circle (2cm);

	\filldraw[shaded] (-1.6,0) arc (180:-180:1.6cm);
	\filldraw[unshaded] (-1.1,0) arc (-180:180:1.1cm);
		
	\draw[ultra thick] (0,0) circle (2cm);

	\node at (0,0)  [Tbox] (T) {$T$};
\end{tikzpicture}

==> Diagrams/Generator/Rotate.tex <==
\begin{tikzpicture}[annular]
\begin{scope}
	\clip (0,0) circle (2cm);

	\filldraw[shaded] (0,0)--(158:2cm) arc (158:112:2cm) -- (0,0);
	\filldraw[shaded] (0,0)--(-158:2cm) arc (-158:-112:2cm) -- (0,0);
	\filldraw[shaded] (0,0)--(22:2cm) arc (22:68:2cm) -- (0,0);
	\filldraw[shaded] (0,0)--(-22:2cm) arc (-22:-68:2cm) -- (0,0);
		
	\draw[ultra thick] (0,0) circle (2cm);

	\node at (0,0)  [Tbox] (T) {$T$};
	\node at (T.180) [left] {$\star$};
\end{scope}
	\node at (90:2cm) [above] {$\star$};
\end{tikzpicture}

==> Diagrams/Generator/Squared.tex <==
\begin{tikzpicture}[scale=.3, inner sep=.5mm, baseline]
	\clip (3,3) arc (0:180:3cm) -- (-3,-3) arc (-180:0:3cm) -- (3,3);
	\filldraw[shaded] (0,3) .. controls ++(-157:3cm) and ++(157:3cm) .. (0,-3) .. controls ++(112:2cm) and ++(-112:2cm) .. (0,3);
	\filldraw[shaded] (0,3) .. controls ++(-22:3cm) and ++(22:3cm) .. (0,-3) .. controls ++(67:2cm) and ++(-67:2cm) .. (0,3);
	\filldraw[shaded] (0,3) -- +(22:4cm) -- +(67:4cm) -- (0,3);
	\filldraw[shaded] (0,3) -- +(112:4cm) -- +(157:4cm) -- (0,3);
	\filldraw[shaded] (0,-3) -- +(-22:4cm) -- +(-67:4cm) -- (0,-3);
	\filldraw[shaded] (0,-3) -- +(-112:4cm) -- +(-157:4cm) -- (0,-3);

	\draw [ultra thick] (3,3) arc (0:180:3cm) -- (-3,-3) arc (-180:0:3cm) -- (3,3);

	\node at (0,3) [Tbox] (T1) {$T$};
	\node at (0,-3) [Tbox] (T2) {$T$};
	\node at (T1.180) [left] {$\star$};
	\node at (T2.180) [left] {$\star$};
	\node at (-3,3) [right] {$\star$};
\end{tikzpicture} 
\in
\operatorname{span}\{ TL, T \}.

==> Diagrams/HighlightSubgraph/Gamma.tex <==
\begin{tikzpicture}[inner sep=2mm, scale=.8]
	\clip (-3.5,-5) rectangle (3.5,6);
	\draw[on] (-150:2cm) .. controls ++(-20:1.5cm) and ++(-160:1.5cm) .. (-30:2cm) -- (-150:2cm);
	\draw[on] (-150:2cm) .. controls ++(20:1.5cm) and ++(160:1.5cm) .. (-30:2cm) .. controls ++(130:1.5cm) and ++(-70:1.5cm) .. (90:2cm) .. controls ++(-90:1.5cm) and ++(30:1.5cm) .. (-150:2cm);
	\draw[on] (-150:2cm) .. controls ++(50:1.5cm) and ++(-110:1.5cm) .. (90:2cm) .. controls ++(-130:1.5cm) and ++(70:1.5cm) .. (-150:2cm);
	\draw[off] (-150:2cm) .. controls ++(90:1.5cm) and ++(-150:1.5cm) .. (90:2cm) .. controls ++(100:1.5cm) and ++(-100:1.5cm) .. (0,5) .. controls ++(-120:3cm) and ++(110:2cm) .. (-150:2cm);
	\draw[off] (-30:2cm) .. controls ++(110:1.5cm) and ++(-50:1.5cm) .. (90:2cm) .. controls ++(80:1.5cm) and ++(-80:1.5cm) .. (0,5) .. controls ++(-60:3cm) and ++(70:2cm) .. (-30:2cm);
	\draw[off] (-30:2cm) .. controls ++(-130:1.5cm) and ++(70:1.5cm) .. (0,-4) .. controls ++(50:1.5cm) and ++(-110:1.5cm) .. (-30:2cm);
	
%redraw some of the edges on
	\draw[on] (-150:2cm) .. controls ++(90:1.5cm) and ++(-150:1.5cm) .. (90:2cm);
	\draw[on] (-30:2cm) .. controls ++(110:1.5cm) and ++(-50:1.5cm) .. (90:2cm);
	
	\draw[off] (0,-4) .. controls ++(150:5cm) and ++(-150:5cm) .. (0,5) .. controls ++(-30:5cm) and ++(30:5cm) .. (0,-4);
	
	\draw[off] (0,-4) -- ++(-45:2cm);
	\draw[off] (0,-4) -- ++(-75:2cm);
	\draw[off] (0,-4) -- ++(-105:2cm);
	\draw[off] (0,-4) -- ++(-135:2cm);
	
	\draw[off] (0,5) -- ++(75:2cm);
	\draw[off] (0,5) -- ++(105:2cm);
	
	\filldraw[on] (-150:2cm) circle (1mm);	
	\filldraw[on] (-30:2cm) circle (1mm);
	\filldraw[on] (90:2cm) circle (1mm);
	\filldraw[off] (0,5) circle (1mm);
	\filldraw[off] (0,-4) circle (1mm);
\end{tikzpicture}

==> Diagrams/HighlightSubgraph/GammaCup.tex <==
\begin{tikzpicture}[inner sep=2mm, scale=.8]
	\clip (-3.5,-5) rectangle (3.5,6);
	\draw[on] (-150:2cm) .. controls ++(-20:1.5cm) and ++(-160:1.5cm) .. (-30:2cm) -- (-150:2cm);
	\draw[on] (-150:2cm) .. controls ++(20:1.5cm) and ++(160:1.5cm) .. (-30:2cm) .. controls ++(130:1.5cm) and ++(-70:1.5cm) .. (90:2cm) .. controls ++(-90:1.5cm) and ++(30:1.5cm) .. (-150:2cm);
	\draw[on] (-150:2cm) .. controls ++(50:1.5cm) and ++(-110:1.5cm) .. (90:2cm) .. controls ++(-130:1.5cm) and ++(70:1.5cm) .. (-150:2cm);
	\draw[on] (-150:2cm) .. controls ++(90:1.5cm) and ++(-150:1.5cm) .. (90:2cm) .. controls ++(100:1.5cm) and ++(-100:1.5cm) .. (0,5) .. controls ++(-120:3cm) and ++(110:2cm) .. (-150:2cm);
	\draw[on] (-30:2cm) .. controls ++(110:1.5cm) and ++(-50:1.5cm) .. (90:2cm) .. controls ++(80:1.5cm) and ++(-80:1.5cm) .. (0,5) .. controls ++(-60:3cm) and ++(70:2cm) .. (-30:2cm);
	\draw[on] (-30:2cm) .. controls ++(-130:1.5cm) and ++(70:1.5cm) .. (0,-4) .. controls ++(50:1.5cm) and ++(-110:1.5cm) .. (-30:2cm);
	
	\draw[off] (0,-4) .. controls ++(150:5cm) and ++(-150:5cm) .. (0,5) .. controls ++(-30:5cm) and ++(30:5cm) .. (0,-4);
	
	\draw[off] (0,-4) -- ++(-45:2cm);
	\draw[off] (0,-4) -- ++(-75:2cm);
	\draw[off] (0,-4) -- ++(-105:2cm);
	\draw[off] (0,-4) -- ++(-135:2cm);
	
	\draw[off] (0,5) -- ++(75:2cm);
	\draw[off] (0,5) -- ++(105:2cm);
	
	\filldraw[on] (-150:2cm) circle (1mm);	
	\filldraw[on] (-30:2cm) circle (1mm);
	\filldraw[on] (90:2cm) circle (1mm);
	\filldraw[on] (0,5) circle (1mm);
	\filldraw[on] (0,-4) circle (1mm);
\end{tikzpicture}

==> Diagrams/HighlightSubgraph/Subgraph.tex <==
\begin{tikzpicture}[inner sep=2mm,scale=.8]
 	\clip (-3.5,-5) rectangle (3.5,6);
	\draw[] (-150:2cm) .. controls ++(-20:1.5cm) and ++(-160:1.5cm) .. (-30:2cm) -- (-150:2cm);
	\draw[] (-150:2cm) .. controls ++(20:1.5cm) and ++(160:1.5cm) .. (-30:2cm) .. controls ++(130:1.5cm) and ++(-70:1.5cm) .. (90:2cm) .. controls ++(-90:1.5cm) and ++(30:1.5cm) .. (-150:2cm);
	\draw[] (-150:2cm) .. controls ++(50:1.5cm) and ++(-110:1.5cm) .. (90:2cm) .. controls ++(-130:1.5cm) and ++(70:1.5cm) .. (-150:2cm);
	\draw[] (-150:2cm) .. controls ++(90:1.5cm) and ++(-150:1.5cm) .. (90:2cm) ..controls ++(100:1.5cm) and ++(-100:1.5cm) .. (0,5) .. controls ++(-120:3cm) and ++(110:2cm) .. (-150:2cm);
	\draw[] (-30:2cm) .. controls ++(110:1.5cm) and ++(-50:1.5cm) .. (90:2cm) .. controls ++(80:1.5cm) and ++(-80:1.5cm) .. (0,5) .. controls ++(-60:3cm) and ++(70:2cm) .. (-30:2cm);
	\draw[] (-30:2cm) .. controls ++(-130:1.5cm) and ++(70:1.5cm) .. (0,-4) .. controls ++(50:1.5cm) and ++(-110:1.5cm) .. (-30:2cm);
	
	\draw (0,-4) .. controls ++(150:5cm) and ++(-150:5cm) .. (0,5) .. controls ++(-30:5cm) and ++(30:5cm) .. (0,-4);
	
	\draw (0,-4) -- ++(-45:2cm);
	\draw (0,-4) -- ++(-75:2cm);
	\draw (0,-4) -- ++(-105:2cm);
	\draw (0,-4) -- ++(-135:2cm);
	
	\draw (0,5) -- ++(75:2cm);
	\draw (0,5) -- ++(105:2cm);
	
	\filldraw (-150:2cm) circle (1mm);	
	\filldraw (-30:2cm) circle (1mm);
	\filldraw (90:2cm) circle (1mm);
	\filldraw (0,5) circle (1mm);
	\filldraw (0,-4) circle (1mm);
\end{tikzpicture}

==> Diagrams/TikzStyles.tex <==
\tikzstyle{shaded}=[fill=red!10!blue!20!gray!30!white]
\tikzstyle{shaded line}=[double=red!10!blue!20!gray!30!white, double distance=2mm, draw=black]
\tikzstyle{unshaded}=[fill=white]
\tikzstyle{unshaded line}=[double=white, double distance=2mm, draw=black]
\tikzstyle{Tbox}=[circle, draw, thick, fill=white, opaque,]
\tikzstyle{background rectangle}= [fill=red!10!blue!20!gray!40!white,rounded corners=2mm] 
\tikzstyle{on}=[very thick, red!50!blue!50!black]
\tikzstyle{off}=[gray]

\tikzstyle{make triple edge size}= [scale=.4, inner sep=1mm,baseline] 
\tikzstyle{icosahedron network}=[scale=.4]
